Neural Visibility Field for Uncertainty-Driven Active Mapping

This paper presents Neural Visibility Field (NVF), a novel uncertainty quantification method for Neural Radiance Fields (NeRF) applied to active mapping. Our key insight is that regions not visible in the training views lead to inherently unreliable color predictions by NeRF at this region, resulting in increased uncertainty in the synthesized views. To address this, we propose to use Bayesian Networks to composite position-based field uncertainty into ray-based uncertainty in camera observations. Consequently, NVF naturally assigns higher uncertainty to unobserved regions, aiding robots to select the most informative next viewpoints. Extensive evaluations show that NVF excels not only in uncertainty quantification but also in scene reconstruction for active mapping, outperforming existing methods.

==> 13_ablation.tex <==

\begin{table*}[htbp]
  \centering
  \caption{Ablation Studies} \label{table:2}
        \begin{tabular}{ccccccccc}
    \toprule
    Ablations & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & RGB$\downarrow$ & Acc.$\downarrow$ & Comp.$\downarrow$ & C.R.$\uparrow$ & Vis.$\uparrow$ \\
    \midrule
    w/o Vis. & 24.98 & 0.856 & 0.185 & 0.0033 & 0.0355 & 0.0209 & 0.405 & 0.332 \\
    w/o Var. & 27.80 & 0.913 & 0.100 & 0.0017 & 0.0202 & 0.0100 & 0.681 & 0.705 \\
    Independent Rays & 25.78 & 0.865 & 0.183 & 0.0027 & 0.0264 & 0.0135 & 0.493 & 0.541 \\
    Loose Bound & 25.81 & 0.910 & 0.110 & 0.0026 & 0.0169 & 0.0128 & 0.630 & 0.603 \\
    NVF (Ours) & 27.99 & 0.919 & 0.100 & 0.0016 & 0.0225 & 0.0110 & 0.651 & 0.681 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> table_gradient.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Performance of gradient-based methods} \label{table:3}
    \begin{tabular}{ccccccccc}
    \toprule
    Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & RGB$\downarrow$ & Acc.$\downarrow$ & Comp.$\downarrow$ & C.R.$\uparrow$ & Vis.$\uparrow$ \\
    \midrule
    AIR   & 24.63 & 0.862 & 0.182 & 0.0035 & 0.0249 & 0.0140 & 0.525 & 0.586 \\
    NeurAR & 25.19 & 0.772 & 0.265 & 0.0030 & 0.0480 & 0.0170 & 0.416 & 0.537 \\
    NVF   & 27.99 & 0.919 & 0.100 & 0.0016 & 0.0225 & 0.0110 & 0.651 & 0.681 \\
    \midrule
    AIR-OPT & 24.41 & 0.858 & 0.183 & 0.0037 & 0.0267 & 0.0159 & 0.450 & 0.548 \\
    NeurAR-OPT & 25.42 & 0.794 & 0.245 & 0.0029 & 0.0461 & 0.0180 & 0.381 & 0.563 \\
    NVF-OPT  & \textbf{29.33} & \textbf{0.930} & \textbf{0.086} & \textbf{0.0012} & \textbf{0.0196} & \textbf{0.0106} & \textbf{0.666} & \textbf{0.690} \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%

